Effective Diversity in Population Based Reinforcement Learning

Exploration is a key problem in reinforcement learning, since agents can only learn from data they acquire in the environment. With that in mind, maintaining a population of agents is an attractive method, as it allows data be collected with a diverse set of behaviors. This behavioral diversity is often boosted via multi-objective loss functions. However, those approaches typically leverage mean field updates based on pairwise distances, which makes them susceptible to cycling behaviors and increased redundancy. In addition, explicitly boosting diversity often has a detrimental impact on optimizing already fruitful behaviors for rewards. As such, the reward-diversity trade off typically relies on heuristics. Finally, such methods require behavioral representations, often handcrafted and domain specific. In this paper, we introduce an approach to optimize all members of a population simultaneously. Rather than using pairwise distance, we measure the volume of the entire population in a behavioral manifold, defined by task-agnostic behavioral embeddings. In addition, our algorithm Diversity via Determinants (DvD), adapts the degree of diversity during training using online learning techniques. We introduce both evolutionary and gradient-based instantiations of DvD and show they effectively improve exploration without reducing performance when better exploration is not required.

==> maintain_div.tex <==
\section{Maintaining a Diverse Population}
\label{adapting_pop}

\textcolor{red}{Key Questions:}

For most of these, the goal is open-endedness rather than sample efficiency. We want to explore in order to find the best possible local optimum. 

\begin{itemize}
    \item How do we ensure the agents in the meta-population are different enough to warrant including them. 
    \item How do we ensure that we do not support a population of badly performing agents just because they are diverse? Trade off: as some may be late bloomers. 
\end{itemize}

The current means to measure population diversity are generally based on the mean pairwise distance in the embedding space. This can trivially lead to a situation whereby policies are clustered together into $k$ clusters ($k>1$), such that the distance between the clusters is high, yet the overall diversity of the population is unlikely to be materially impacted if the clusters reduced to a single policy. This is not only a waste of compute, since multiple similar policies may be maintained, but also may prevent exploration in additional areas of the parameter space. 

Furthermore, the current means to balance the reward and novelty is based on heuristics. For example, in NSR-ES, $\beta$ is simply set to $0.5$. The authors of \cite{novelty} also proposed an adaptive scheme NSRA-ES, which initializes $\beta$ to be zero and gradually increases it throughout optimization, yet fails to ensure the two objectives do not offset one another at each step (and is also based on some heuristics...). 

Our proposed approach seeks address both these issues. We have yet to decide upon the exact methodology, however below are some presented ideas:
\begin{itemize}
    \item \textbf{Alternating Optimization} We optimize the population for reward for $k$ steps, then do one update to maximize the determinant of the embeddings of all policies. This can be done by perturbing all the policies by a small amount in a way that maximizes the determinant of the $M$ embeddings. 
    \item \textbf{Diversity-Driven} Similar to above, we can optimize for reward, but switch to diversity for $1$ step if it is required (rather than a pre-meditated decision). \textit{Required} here needs to be defined rigorously! 
    \item \textbf{Joint Optimization} We can also optimize the whole population at once, by considering one perturbation vector $\epsilon \in \mathbb{R}^{Md}$. The benefit of this approach is that we can optimize for both determinant of the kernel matrix as well as mean reward across the population. This has been tested on small environments and as of yet has not worked. 
    \item \textbf{Replacing Agents} One weakness of Dive-In may be that we initialize overly negative behaviors. Therefore, it may be worthwhile replacing the bottom performing members of the population. Rather than using a heuristic, it would be interesting to conceive a more rigorous means to decide this (I will do some reading in the literature). Once deleted, we can decide to add the new agent by perturbing the best performing agent and then selecting the one which maximizes the determinant of the kernal matrix with the other $M-1$ agents. 
    \item \textbf{Re-Defining Novelty} We simply use the same construction as NSR-ES but calculate novelty as the determinant of the kernel matrix of each sample's embedding and the remaining $M-1$ agents. The most incremental idea here.
    \item \textbf{Adapt Population Size} We could use this mechanism to adapt the size of $M$, which was shown to be effective by this DeepMind paper \cite{Malthusian}.
    \item \textbf{Use Probabilistic Embeddings} This would make embeddings incorporate some stochasticity in embeddings, would require using Wasserstein Distances (or some other distance on probability distributions). 
\end{itemize}

In addition, we should consider the mechanism for sampling policies, incorporating the maximum reward obtained by the policy, in order to fix the problem of consistently using compute on poor performing agents simply because they are diverse. This resembles a multi-armed bandit and instantiates an exploration problem itself!

\begin{comment}
DPPs, as previously introduced, can be used to measure the total volume of the space spanned by a set of policies $\pi_{\theta_1}, \dots, \pi_{\theta_M}$. We know that the diversity of the population can be measured as the determinant of the kernel matrix of the policy embeddings, $\Phi(\theta_1) \dots, \Phi(\theta_M)$.
\begin{definition}\label{Def:behav_div} \textbf{(Behavioral Diversity Score)} We define the behavioral diversity score (BDS) of a population as $det(\mathbf{K})$ where $\mathbf{K}$ is a kernel matrix of the policy embeddings $\Phi(\theta_1), \dots, \Phi(\theta_M)$.
\end{definition}
This idea leads to the following:\begin{definition}\label{Def:incremental} \textbf{(Incremental Population Diversity)}
Let $\mathcal{X} = \Phi(\theta_1), \dots, \Phi(\theta_M)$ be a population of embeddings for policies parameterized by $\theta_1, \dots, \theta_M$, and $\mathbf{K}$ be a kernel matrix of these embeddings. Let $A = \mathcal{X} - \{\Phi(\theta_i)\}$, and $\mathbf{K}_{A}$ be be the submatrix of $\mathbf{K}$ indexed by elements of A. We define the incremental diversity of policy $i$ as: $det(\mathbf{K}) - det(\mathbf{K}_{A})$ \end{definition}
\end{comment}




==> motivation.tex <==
\section{Motivating Diversity via Determinants}
\label{sec:determinants}

\vspace{-4mm}
\begin{figure}[h]
  \centering
	\includegraphics[keepaspectratio, width=0.5\textwidth]{plots/fin3.png}
  \caption{Illustration of problems with standard novelty search exploration. (a): populations of agents split into four clusters with agents within cluster discovering similar policies. (b): embedded policies $\Phi(\theta_{1}),...,\Phi(\theta_6)$ lay in a grey hyperplane. In (a) resources within a cluster are wasted since agents discover very similar policies. In (b) all six embeddings can be described as linear combinations of embeddings of fewer canonical policies. In both settings standard novelty techniques assign high novelty scores but diversity as measured by determinants is low.}
\vspace{-2mm}  
\label{fig:dependent_updates}  
\end{figure}

Choosing determinants to quantify diversity is crucial. First of all, they prevent the undesirable clustering phenomenon, where a population evolves to a collection of conjugate classes, that standard distance-based methods are not resilient to. To illustrate this point, consider a simple scenario, where all $M$ agents are partitioned into $k$ clusters of size $\frac{M}{k}$ each for $k=o(M)$. By increasing the distance between the clusters one can easily make the novelty measured as an average distance between agents' embedded policies as large as desired, but that is not true for the corresponding determinants which will be zero if the similarity matrix is low rank. Furthermore, even if all pairwise distances are large, the determinants can be still close to zero if spaces where agents' high-dimensional policy embeddings live can be accurately approximated by much lower dimensional ones. Standard methods are too crude to measure novelty in such a way (see: Fig. \ref{fig:dependent_updates}).

From a geometric perspective, the determinant of the kernel matrix represents the volume of a parallelepiped spanned by feature maps corresponding to the kernel choice. We seek to maximize this volume, effectively ``filling'' the feature (or behavior) space. 

Another interpretation as to why this may be effective is the ability for $\mathrm{DvD}$ to reason one step ahead. Typical novelty search methods assume the remaining members of the population are static. When these agents subsequently move in the behavior space they can induce cycling since the agents are constantly trying to repel from one another. For $\mathrm{DvD}$, each agent has the joint objective of maximizing the population diversity, and thus can consider the changing behavior of all agents simultaneously.   
